Warm, not Fuzzy: Generalized Ultralight Dark Matter Limits from Milky Way Satellites

We generalize lower limits on the dark matter (DM) particle mass $m$ derived from Milky Way (MW) satellite galaxy abundances to scenarios in which DM is an ultralight scalar field produced with a field power spectrum peaked at a subhorizon wavenumber $k_*$. In these models, the DM field free-streams similarly to warm DM while also exhibiting significant small-scale wave interference effects. The resulting dimensionless density power spectrum shows two effects: (i) free-streaming suppression at $k_{\rm fs}\sim k_{\rm eq}/[(k_*/a_{\rm eq}m)\ln(a_{\rm eq}m/k_*)]$; (ii) Poisson-like enhancement related to wave interference at $k\gtrsim10^{-2}k_*$, which saturates near the Jeans scale $k_{\rm J}\sim k_{\rm eq}/(k_*/a_{\rm eq}m)$. Comparing these predictions with established constraints on a free-streaming cutoff in the linear matter power spectrum from the MW satellite population and assuming that warm ultralight DM does not change the form of the galaxy--halo connection relative to cold DM, we obtain $m>6\times10^{-18}\,{\rm eV}\,(k_*/10^4\,{\rm Mpc}^{-1})$ for $k_*>10^4\,{\rm Mpc}^{-1}$ at 95% confidence. For smaller $k_*$, Poisson-noise enhancement on MW satellite scales weakens the constraint, yielding $m>6\times10^{-18}\,{\rm eV}\,(k_*/10^4\,{\rm Mpc}^{-1})^2$ for $k_*<10^4\,{\rm Mpc}^{-1}$ at 95% confidence.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

